3D-LDM: Neural Implicit 3D Shape Generation with Latent Diffusion Models

Diffusion models have shown great promise for image generation, beating GANs in terms of generation diversity, with comparable image quality. However, their application to 3D shapes has been limited to point or voxel representations that can in practice not accurately represent a 3D surface. We propose a diffusion model for neural implicit representations of 3D shapes that operates in the latent space of an auto-decoder. This allows us to generate diverse and high quality 3D surfaces. We additionally show that we can condition our model on images or text to enable image-to-3D generation and text-to-3D generation using CLIP embeddings. Furthermore, adding noise to the latent codes of existing shapes allows us to explore shape variations.

==> supplementary_sections/applications.tex <==

\begin{figure*}[t]
  \centering
\includegraphics[width=\linewidth,height=0.5\linewidth]{sections/imgs/exploration.pdf}
  \caption{Guided shape exploration. By adding noise to the input shape (left column), we can generate variations of the input shapes that can be used for shape exploration. In each column we show a different generated sample after adding 2000 noise steps to the input shape. We can see that the coarse shape of the input is preserved, but each variation generates different shape detail.}
  \label{fig:exploration}
\end{figure*}

\section{Shape Exploration}
\label{sec:applications}

In this section, we show qualitative results for the shape exploration application mentioned in the main paper. We can explore variations of a given input shape by adding noise to its latent vector and denoising it using our method. The amount of noise controls how similar the generated shape variations are to the input shape. In Figure~\ref{fig:exploration} shows generated variations for three input shapes. The number of noise steps has to be big enough so that the denoising process does not deterministically trace the original shape back and not too big to avoid generating random shapes unrelated to the shape of origin. For our experiments, we add 2000 noise steps and denoise using our method for the same number of steps. We can see that the shape variations explore different shape detail, while preserving the coarse shape of the input.


==> supplementary_sections/applications_bis.tex <==
\section{CLIP Conditioning}
\label{sec:applications2}

In Figure~\ref{fig:textclip} and Figure~\ref{fig:imclip}, we showcase the versatility of our method by extending it to a conditioning based on CLIP-embeddings~\cite{radford2021learning}. By training a version of \name conditioned on shape renderings encoded through CLIP, we not only allow for shape generation through images which were used for the training part but also text prompts thanks to the common domain  of the text and image embddings in CLIP. For our text-to-shape experiments, we use more descriptive and implicit text such as \textit{"This is a spinning chair with wheels"} instead of the category-based text \textit{"This is an office chair"}. Through the results, we can see that \name conditioned on CLIP embeddings yields reasonable results for both image and text inputs.

\begin{figure}[t]
  \centering
\includegraphics[width=\linewidth]{sections/imgs/textclip.pdf}
  \caption{Text-to-Shape. \name conditioned on CLIP embeddings can generate shapes that match the description given by the text prompt. In each row, we showcase multiple shapes generated by our model for each text prompt.}
  \label{fig:textclip}
\end{figure}

\begin{figure}[t]
  \centering
\includegraphics[width=\linewidth]{sections/imgs/imgclip.pdf}
  \caption{Image-to-Shape. \name conditioned on CLIP embeddings can generate shapes similar to an input image. In each row, we showcase multiple shapes generated by our model for two different image renderings of chairs extracted from the \textit{chairs} dataset.}
  \label{fig:imclip}
\end{figure}


